PARIS: Personalized Activity Recommendation for Improving Sleep Quality

The quality of sleep has a deep impact on people's physical and mental health. People with insufficient sleep are more likely to report physical and mental distress, activity limitation, anxiety, and pain. Moreover, in the past few years, there has been an explosion of applications and devices for activity monitoring and health tracking. Signals collected from these wearable devices can be used to study and improve sleep quality. In this paper, we utilize the relationship between physical activity and sleep quality to find ways of assisting people improve their sleep using machine learning techniques. People usually have several behavior modes that their bio-functions can be divided into. Performing time series clustering on activity data, we find cluster centers that would correlate to the most evident behavior modes for a specific subject. Activity recipes are then generated for good sleep quality for each behavior mode within each cluster. These activity recipes are supplied to an activity recommendation engine for suggesting a mix of relaxed to intense activities to subjects during their daily routines. The recommendations are further personalized based on the subjects' lifestyle constraints, i.e. their age, gender, body mass index (BMI), resting heart rate, etc, with the objective of the recommendation being the improvement of that night's quality of sleep. This would in turn serve a longer-term health objective, like lowering heart rate, improving the overall quality of sleep, etc.

==> 2background.tex <==

The quality of sleep has a deep impact on people's physical and mental health. Good sleep can keep a person active and fresh whereas poor sleep can lead to drowsiness, headache, and lethargy. ~\citep{strine2005associations} show that insufficient sleep is related to health-related quality of life and health behaviors. 
People with insufficient sleep are more likely to report physical and mental distress, activity limitation, anxiety, and pain. Decreased sleep duration or quality may increase diabetes risk ~\citep{knutson2006role}, severe cardiovascular consequences~\citep{kasasbeh2006inflammatory}, depression~\citep{murphy2015sleep}, etc. 
%A study~\cite{williamson2000moderate} shows that moderate deprivation of sleep affects the cognitive and motor performance of a person in the same way as alcohol does. Because of the great impact of sleep in people's overall well-being, sleep science has become an active research area in recent years.
Two recent studies \citep{blume2020effects, wright2020sleep} have shown how movement restrictions imposed due to COVID-19 led to an increase in sleep duration but lowering of the quality of sleep because of an increase in perceived burden.

Because of the impact of sleep on public health, and the increase in the number of people with sleep-related diseases, large companies like Apple, Google, Samsung, Fitbit along with start-ups are investing in sleep technology and sleep-related research. Polysomnography (PSG), a test to diagnose sleep disorder, was developed in 1950s~\citep{hirshkowitz2015history}. It records brain waves, the oxygen level in the blood, heart rate, and breathing, as well as eye and leg movements during the test.
%PSG measures brain activity, eye movements, muscle activity, and heart rhythm. 
But the test has to be done in a sleep lab or hospital. Since PSG is a high-fidelity test, it is considered a gold standard for sleep research. But PSG is not scalable, it is too expensive and it does not consider physical activity during the day. %As a result, PSG cannot be used as a common tool to identify sleep disorders and to improve sleep quality.

%As an alternative to PSG, %which can only be performed in sleep lab which might lead to inconvenience for many people,
%a new technology emerged in the 1990s, known as Home Sleep Test (HST)~\cite{douglas2003home}. Patients could then carry out the test at home using a small device. Although it is much more affordable than PSG, it had a limited application in diagnosing sleep apnea. %With the emergence of wearable devices, a solution was found to both of the problems: affordability and effectiveness. 

There have been various studies that have shown how the activities carried out during the day could affect sleep. A study~\citep{kredlow2015effects} shows the impact of different exercise levels on different stages of sleep, sleep time, and sleep efficiency. ~\citep{chennaoui2015sleep} discuss how sleep and exercise influence each other: how different physical activity levels influence physical stages during sleep, and how sleep quality influences exercise performance. Other studies demonstrated that a certain amount of exercise helps to reduce insomnia~\citep{yang2012exercise, merrill2007effects} and sleep apnea~\citep{awad2012exercise}. 
All of these studies conducted their experiment on particular groups of people using direct monitoring, surveys, questionnaires, or using PSG. %So it is not possible for a person staying at home to know whether he is going to have a good sleep or not

With the advent of the Quantified Self movement~\citep{swan2009qs}, which %represents the entry of big data in the domain of measuring personal information. The movement focuses on collecting and analyzing data about oneself with the objective of improving productivity and the health of individuals, there has been an explosion of applications and devices for activity monitoring and health tracking. 
% Health component of the movement has shown so much promise for widespread adoption and market potential, that now this movement is perceived as only about health. 
The products available are getting more sophisticated and can track a wide array of things, like heart rate, sleep patterns, steps taken, and provide analysis and feedback on how these can be improved to lead a healthier life. These self-tracking devices have empowered people to monitor their health proactively and be able to take appropriate measures to alleviate possible health risks. 

Moreover, signals collected from these wearable devices can be used to study sleep quality and sleep disorders. There have been numerous studies that have validated the use of wrist-worn devices to estimate sleep ~\citep{cole92,jean01b,quante18,smith2018use} and even compared the data with PSG, with satisfying results.

Along with this progress in the health domain, there has been a great deal of progress in the computing domain for efficiently processing huge amounts of data. The evolution of machine learning and deep learning techniques is transforming the field of sleep medicine as new techniques are continually emerging \citep{hossain2018active}. 

%Furthermore, there are initiatives like \url{sleepdata.org} by the National Sleep Research Resource (NSRR), that allow researchers to freely access data from clinical trials~\cite{dean16,zhang18}, as well as tools to experiment with the data. 

This immense body of work in the domain of wearable devices and sleep tracking motivated us to study the relationship between physical activity and sleep quality using machine learning techniques, and to find ways of assisting people in improving their sleep. 
%% Meghna: add background on rec sys
Furthermore, most of the existing fitness tracking applications provide generic recommendations to consumers for helping them achieve their health goals, usually based on gender and age. The “one-size-fits-all” principle doesn't necessarily fulfill the health objectives of many people. There is a growing need for more personalized advice based on users’ health goals, environment, and daily activities along with the existing body metrics like age, gender, and BMI. Personalization is critical for providing effective recommendations (i.e. achieving required behavioral change) as the state of health, level of self-control, physical activity types, duration of those activities and timing would be different for each subject.




==> declaration.tex <==
This paper or a similar version is not currently under review by a journal or conference. This paper is void of plagiarism or self-plagiarism as defined by the Committee on Publication Ethics and Springer Guidelines.


4. What are the main limitations of your approach?
One of the main limitations of our approach is the difficulty to test the approach in real-time, as opposed to retrospective analysis that we had to carry out. In a real-time system we could get feedback, which would help in improving the recommendations, but that is not possible in the current scenario.



----
1. What is the scientific question you are addressing? What are the key findings that answer this question? Why is this work important and timely? Why is it of interest to the readership of this journal? Please provide below a statement explaining the significance of this submission.

Our submission addresses the question of the type of activity recommendation to be made for a user based on his activities thus far, while also adhering to the user's health and lifestyle constraints, with the objective of improving sleep. This work is important because health is a domain where consequences of incorrect recommendations can be very significant, both immediately as well as long term. So it is necessary that the health of the subject be taken into consideration before suggesting activities for improving their lifestyle. Moreover, with the current situation of the world, irregular schedules and stress are on the rise, which in turn affect sleep quality. So our work is a step in the right direction of helping people find ways that are easy to adopt and match their health status. 
This journal particularly is on recommender systems for health and well being, so our work is very well aligned to the objectives of the special issue.
We  present  a  novel  approach  for  goal-directed  personalized activity recommendations that finds activities most closely aligned with a user based on activities done thus far, as well as any health constraints the user might have.

2. What is the relationship of your work to the closest 2-3 publications by others? (also cite them)

(Nosakhare andPicard, 2020) is closest to our work as they used machine learning models for finding days similar to an existing day for a subject, and used those to make recommendations about changes in behaviors that would result in achieving an end goal, which in their case was lowering stress.

(Alcaraz-Herrera and Palomares, 2019) recommend food and exercise bundles to users based on their preferences and health goals, which is similar to our work in that the users' preferences are taken into account.

Ni  et  al,  2019   present   personalized  systems for recommending workout routes based on user preferences and health profiles, and this work is close to our work in the personalized recommendation aspect.

1. Nosakhare E, Picard R (2020) Toward assessing and recommending combina-tions of behaviors for improving health and well-being. ACM Transactionson Computing for Healthcare 1(1):1–29
2. Alcaraz-Herrera H, Palomares I (2019) Evolutionary approach for’healthy bun-dle’wellbeing recommendations
3. Ni J, Muhlstein L, McAuley J (2019) Modeling heart rate and activity data forpersonalized fitness recommendation. In: The World Wide Web Conference,ACM, pp 1343–1353


3. Why does your planned submission fit into the scope of UMUAI?
Our submission specifically aims at addressing the issue of personalized recommendations for health and well-being, which makes it closely aligned to this journal's scope.

